Improving VTE Identification through Adaptive NLP Model Selection and Clinical Expert Rule-based Classifier from Radiology Reports

Rapid and accurate identification of Venous thromboembolism (VTE), a severe cardiovascular condition including deep vein thrombosis (DVT) and pulmonary embolism (PE), is important for effective treatment. Leveraging Natural Language Processing (NLP) on radiology reports, automated methods have shown promising advancements in identifying VTE events from retrospective data cohorts or aiding clinical experts in identifying VTE events from radiology reports. However, effectively training Deep Learning (DL) and the NLP models is challenging due to limited labeled medical text data, the complexity and heterogeneity of radiology reports, and data imbalance. This study proposes novel method combinations of DL methods, along with data augmentation, adaptive pre-trained NLP model selection, and a clinical expert NLP rule-based classifier, to improve the accuracy of VTE identification in unstructured (free-text) radiology reports. Our experimental results demonstrate the model's efficacy, achieving an impressive 97\% accuracy and 97\% F1 score in predicting DVT, and an outstanding 98.3\% accuracy and 98.4\% F1 score in predicting PE. These findings emphasize the model's robustness and its potential to significantly contribute to VTE research.

==> background.tex <==
\section{Background} \label{background}
\subsection{Transfer Learning}
Transfer learning is a machine learning technique that involves leveraging knowledge gained from pretraining a model on one task to improve performance on a different task. It has been particularly effective in the field of NLP with the advent of pre-trained models like BERT (Bidirectional Encoder Representations from Transformers). BERT models have been trained on large-scale corpora: Wikipedia 2.5 billion words and Books Corpus 0.8 billion words, using unsupervised learning. These models learn contextualized word representations, capturing the relationships and meanings of words within a sentence. 

In transfer learning using BERT, the pre-trained model's knowledge is transferred to a downstream task by fine-tuning the model on a smaller labeled dataset specific to that task. This allows the model to benefit from the pre-trained representations and learn task-specific patterns from the limited labeled data. By utilizing pre-trained BERT models in transfer learning, NLP tasks such as text classification can be performed more effectively, even with limited labeled data. The contextualized word embeddings captured by BERT improve the model's ability to understand and generate meaningful representations of text, leading to enhanced performance on a wide range of NLP tasks.

\subsection{Data Augmentation}
The Deep Learning research community is actively investigating various approaches to address the challenge of learning without labeled big data. Alongside Transfer Learning, self-supervised learning and Data Augmentation (DA) have shown promising results in this endeavor. DA is one of the most useful techniques to enhance the training of Deep Neural Networks \cite{shorten2021text}. Text DA is also a valuable approach for addressing data imbalance in NLP tasks. It can help mitigate the issue by generating additional synthetic examples. DA involves applying various transformations or modifications to the original text while preserving its meaning and context.  

DA is a widely employed technique in computer vision (CV), where methods like cropping, flipping, and color jittering are commonly used during model training. However, in NLP tasks, generating effective augmented examples that capture the desired invariances is not as straightforward due to the discrete nature of the input space \cite{feng2021survey}. Numerous data augmentation techniques have been proposed for NLP, despite the inherent challenges posed by text data. Empirical study \cite{chen2023empirical} demonstrates that: in supervised learning, token-level augmentations, particularly word replacement and random swapping, consistently show the highest improvement in performance. On the other hand, in semi-supervised learning, sentence-level augmentation, specifically round-trip translation, demonstrates the most significant improvement in performance. In both supervised and semi-supervised settings, token-level augmentations and sentence-level augmentations are generally considered more dependable than hidden-level augmentations. However, the effectiveness of DA depends on the datasets and tasks \cite{cubuk2019autoaugment}, which require a lot of experiments. The investigation of methods for automatically selecting suitable types of data augmentation remains limited.  

\subsection{Word Embedding}
Word embedding is a technique used in NLP to represent words or phrases as dense vectors in a continuous vector space.
% context-free vs contextual
Context-free models such as word2vec \cite{mikolov2013efficient} or GloVe \cite{pennington2014glove} generate a single embedding representation for each word in the vocabulary. Contextual models like BERT \cite{devlin2018bert} instead generate a representation of each word that is based on the other words in the sentence. 
BERT (Bidirectional Encoder Representations from Transformers) improves upon previous models such as Semi-supervised Sequence Learning \cite{dai2015semi}, Generative Pre-Training \cite{radford2018improving}, and ELMo \cite{DBLP:journals/corr/abs-1802-05365} by introducing deep bidirectionality and unsupervised learning. BERT is a powerful Deep Learning model. It is based on the Transformer \cite{vaswani2017attention} architecture, which is a type of neural network model that revolutionized the field of natural language processing. The Transformer architecture utilizes self-attention mechanisms to capture contextual relationships between words or tokens in a sequence. BERT is designed to generate high-quality contextualized word representations by training on large-scale unlabeled text data.
It learns to predict missing words or sentences within a given context, resulting in a deep understanding of language semantics. This pretraining process enables BERT to capture intricate linguistic patterns and relationships, making it effective for a wide range of NLP tasks.

The attention mechanism is a key component in transformers. The attention mechanism allows the transformer to weigh the relevance of different parts of the input sequence when generating its output. In transformers, the attention mechanism operates by computing attention scores between each input element and every other element in the sequence. These attention scores represent the importance or relevance of each element with respect to the others. The attention mechanism then combines these scores with the corresponding values to compute a weighted sum, which is used to create a context vector that captures the important information from the input sequence. The attention mechanism in transformers enables the model to capture long-range dependencies and contextual information from the input sequence. It allows the model to focus on the most relevant parts of the sequence when generating predictions or representations, leading to improved performance in NLP tasks.

==> sections/background.tex <==
%\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/us-class.png} 
    \caption{} 
    \label{fig7:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/us-length.png} 
    \caption{} 
    \label{fig7:b} 
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/ct-class.png} 
    \caption{} 
    \label{fig7:c} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/ct-length.png} 
    \caption{} 
    \label{fig7:d} 
  \end{subfigure} 
  \caption{(a) The pie diagram illustrates the distribution of classes in the dataset of Ultrasound reports, with the ”No DVT” class representing the majority, accounting for 78\% of the reports. (b), A histogram of the number of words in ultrasound reports. The reports in DVT dataset vary in length, ranging from a few words to around 170 words. (c) The pie diagram illustrates the distribution of classes in the dataset of CT scan reports, with the ”No PE” class representing the majority, accounting for 88\% of the reports. (d) A histogram of the number of words in CT scan reports. The reports in PE dataset vary substantially in length, ranging from 100 words to over 600 words.}
  \label{fig:data} 
%\end{figure}
